Capturing vertical information in radially symmetric flow using hyperbolic shallow water moment equations

Models for shallow water flow often assume that the lateral velocity is constant over the water height. The recently derived shallow water moment equations are an extension of these standard shallow water equations. The extended models allow for vertical changes in the lateral velocity, resulting in a system that is more accurate in situations where the horizontal velocity varies considerably over the height of the fluid. Unfortunately, already the one-dimensional models lack global hyperbolicity, an important property of partial differential equations that ensures that disturbances have a finite propagation speed. In this paper we show that the loss of hyperbolicity also occurs in two-dimensional axisymmetric systems. First, a cylindrical moment model is obtained by starting from the cylindrical incompressible Navier-Stokes equations. We derive two-dimensional axisymmetric Shallow Water Moment Equations by imposing axisymmetry in the cylindrical model. The loss of hyperbolicity is observed by directly evaluating the propagation speeds and plotting the hyperbolicity region. A hyperbolic axisymmetric moment model is then obtained by modifying the system matrix in analogy to the one-dimensional case, for which the hyperbolicity problem has already been observed and overcome. The new model is written in analytical form and we prove that hyperbolicity can be guaranteed. To test the new model, numerical simulations with both discontinuous and continuous initial data are performed. We show that the hyperbolic model leads to less oscillations than the non-hyperbolic model in the case of a discontinuous initial height profile. The hyperbolic model is preferred over the non-hyperbolic model in this specific scenario for shorter times. Further, we observe that the error decreases when the order of the model is increased in a test case with smooth initial data.

==> axisymmetric/backup.tex <==
In \cite{Bauerle_Rotational}, it is claimed that the matrix \(A_{HA}^{(N,N)}\) is diagonalizable with real eigenvalues. However, the proof in this paper only holds if \(\alpha_1 \neq 0\). We will now derive the eigenvalues of \(A_{HA}^{(N,N)}\). In particular, the system matrix is a block lower triangular matrix, simplifying the computation of the characteristic polynomial and the eigenvalues below. 

\begin{theorem}\label{22OrderCharPol}
The HASWME system matrix \(A_{HA}^{(N,N)}\in \mathbb{R}^{(N+3)\times (N+3)}\) has the following characteristic polynomial:
\begin{equation}\label{22charpol}
    \chi_{A_{HA}^{(N,N)}}(\lambda)=\left( \left( \lambda -v_{r,m})^2-gh-\alpha_1^2 \right) \right)\cdot \chi_{A_2^{(N,N)}}(\lambda -v_{r,m})\cdot\chi_{A_3^{(N,N)}}(\lambda),
\end{equation}
where \(A_2^{(N,N)}\in \mathbb{R}^{N\times N}\) and \(A_3^{(N,N)}\in \mathbb{R}^{(N+1)\times (N+1)}\) are defined as
\begin{equation*}
    A_2^{(N,N)}=
    \begin{pmatrix}
        &  c_1 & &  \\[6pt]
        a_2 & & \ddots &  \\[6pt]
        & \ddots & & c_{N-1} \\[6pt]
        & & a_{N} &
    \end{pmatrix}, \qquad
    A_3^{(N,N)}=
    \begin{pmatrix}
        v_{r,m} & \frac{\alpha_1}{3} & &  \\[6pt]
        \alpha_1 & v_{r,m} & g_1 & & \\[6pt]
        & f_2 & v_{r,m} & \ddots &  \\[6pt]
        & & \ddots & \ddots & g_{N-1} \\[6pt]
        & & & f_N & v_{r,m}
    \end{pmatrix}
\end{equation*}
with
\begin{align*}
    a_i&=\frac{i-1}{2i-1}\alpha_1, \quad f_i=\frac{i}{2i-1}\alpha_1, \qquad i=2,\ldots,N,\\[5pt]
    c_i&=\frac{i+2}{2i+3}\alpha_1, \quad g_i=\frac{i+1}{2i+3}\alpha_1, \qquad i=1,\ldots,N-1.
\end{align*}
\end{theorem}

\begin{proof}
The characteristic polynomial of the modified system matrix \(A_H^{(N,N)}\) is by definition 
\begin{equation*}
    \chi_{A_{HA}^{(N,N)}}(\lambda)=\det(A_{HA}^{(N,N)}-\lambda I) :=\lvert A_{HA}^{(N,N)}-\lambda I \rvert.
\end{equation*}

Recall that the system matrix has the following form:
\begin{equation*}
    A_{HA}^{(N,N)}=
    \begin{pmatrix}
        \mathbf{A^{(N,N)}} & \mathbf{0} \\
        \mathbf{B^{(N,N)}} & \mathbf{C^{(N,N)}}
    \end{pmatrix},
\end{equation*}
where the explicit form of the blocks \(\boldsymbol{A^{(N,N)}},\boldsymbol{B^{(N,N)}}\) and \(\boldsymbol{C^{(N,N)}}\) is given in Theorem \ref{NNOrderTheoremMatrixForm}. This is a lower triangular block matrix. It is known that the determinant of a triangular block matrix is given by the determinant of its diagonal blocks, see e.g. \cite{silvester_determinants_2000}. So we have:
\begin{equation*}
\lvert A_{HA}^{(N,N)}-\lambda I \rvert =\lvert \boldsymbol{A^{(N,N)}}-\lambda I \rvert \cdot \lvert \boldsymbol{C^{(N,N)}}-\lambda I \rvert.
\end{equation*}

According to \cite{SWME}, the first factor yields:
\begin{equation*}
    \lvert \boldsymbol{A^{(N,N)}}-\lambda I \rvert=\left( \left( \lambda -v_{r,m})^2-gh-\alpha_1^2 \right) \right)\cdot \chi_{A_2^{(N,N)}}(\lambda -v_{r,m}).
\end{equation*}
The observation that \(\boldsymbol{C^{(N,N)}}\) is exactly the matrix \(A_3^{(N,N)}\) as defined above completes the proof.
\end{proof}

\begin{lemma}\label{LemmaDADInverse}
    Let \(A\in \mathbb{R}^{n\times n}\) and \(D=diag(d_1,\cdots,d_n)\in\mathbb{R}^{n\times n}\), with \(d_i\neq 0\) (\(i=1,\cdots,n\)). Then \(A\) and \(DAD^{-1}\) have the same eigenvalues. 
\end{lemma}

\begin{proof}
The proof can be found in Appendix \ref{ch:hyperbolicityproof(N,N)}.
\end{proof}

\begin{lemma}\label{LemmaSymmetric}
Let \(A\in \mathbb{R}^{n\times n}\) be a real tridiagonal matrix such that \(a_{i,i+1}a_{i+1,i}>0\), \(i=1,\ldots,n-1\). Then there is a real diagonal matrix \(D\) such that \(DAD^{-1}\) is symmetric.
\end{lemma}

\begin{proof}
The proof can be found in Appendix \ref{ch:hyperbolicityproof(N,N)}.
\end{proof}

\begin{theorem}\label{theorem:eigenvaluesNN}
The eigenvalues of the modified axisymmetric hyperbolic system matrix \(A_{HA}^{(N,N)} \in \mathbb{R}^{(2N+3)\times (2N+3)}\) are the real numbers

\begin{align}
    \lambda_{1,2}&=v_{r,m}\pm \sqrt{gh+\alpha_1^2},\\[5pt]
    \label{eigenvalues1}\lambda_{i+2}&=v_{r,m}+b_i\alpha_1, \qquad i=1,\ldots,N,\\[5pt]
    \label{eigenvalues2}\lambda_{i+2+N}&=v_{r,m}+s_i\alpha_1,\qquad i=1,\ldots,N+1,
\end{align}
with \(b_i \cdot \alpha_1\) the real roots of \(A_2^{(N,N)}\), and \(s_i \cdot \alpha_1\) the real roots of \(A_3^{(N,N)}\), from Theorem \ref{22OrderCharPol} and where all the \(b_i\)'s are pairwise distinct and where all the \(s_i\)'s are pairwise distinct.
\end{theorem}

\begin{proof}
Recall that the characteristic polynomial of \(A_{HA}^{(N,N)}\) is given by
\begin{equation*}
    \chi_{A_{HA}^{(N,N)}}(\lambda)=\left( \left( \lambda -v_{r,m})^2-gh-\alpha_1^2 \right) \right)\cdot \chi_{A_2^{(N,N)}}(\lambda -v_{r,m})\cdot \chi_{A_3^{(N,N)}}(\lambda).
\end{equation*}

From the first factor, we easily obtain
\begin{equation*}
    \lambda_{1,2}=v_{r,m}\pm \sqrt{gh+\alpha_1^2}.
\end{equation*}

In \cite{SWME}, it is shown that the roots of \(\chi_{A_2^{(N,N)}}(\lambda-v_{r,m})\) have the form \(\lambda_i=v_{r,m}+b_i\cdot \alpha_1\). Moreover, it is proved in \cite{equilibriumStability} that the roots are real.

It remains to prove that the eigenvalues of the matrix \(A_3^{(N,N)}\) are real. For \(\alpha_1=0\), it is obvious that all the eigenvalues are real. If \(\alpha_1\neq0\), it follows from Lemma \ref{LemmaDADInverse} that there is a real diagonal matrix \(D\) such that \(DAD^{-1}\) is symmetric. Since a symmetric matrix has real eigenvalues, it follows from Lemma \ref{LemmaSymmetric} that all the eigenvalues of \(A_3^{(N,N)}\) are real. This completes the proof.
\end{proof}

Finally, we state the following result proved in \cite{Bauerle_Rotational}:

\begin{theorem}
    If \(\alpha_1\neq0\), then the \((N,N)\)th order HASWME are globally hyperbolic.
\end{theorem}

\begin{proof}
    Proved in \cite{Bauerle_Rotational}.
\end{proof}


To show that the eigenvalues of the characteristic polynomial \eqref{NNcharpol_Verbiest} are real, the following lemma is needed.

\begin{lemma}\label{LemmaSymmetric}
Let \(A\in \mathbb{R}^{n\times n}\) be a real tridiagonal matrix such that \(a_{i,i+1}a_{i+1,i}>0\), \(i=1,\ldots,n-1\). Then there exists a real diagonal matrix \(D\) such that \(DAD^{-1}\) is symmetric.
\end{lemma}

\begin{proof}
The proof can be found in Appendix \ref{ch:hyperbolicityproof(N,N)}.
\end{proof}

\begin{replemma}{LemmaSymmetric}
Let \(A\in \mathbb{R}^{n\times n}\) be a real tridiagonal matrix such that \(a_{i,i+1}a_{i+1,i}>0\), \(i=1,\ldots,n-1\). Then there is a real diagonal matrix \(D\) such that \(DAD^{-1}\) is symmetric.
\end{replemma}

\begin{proof}
We will construct a diagonal matrix \(D\) such that \(DAD^{-1}\) to prove the theorem. Let 
\begin{equation*}
    D=
    \begin{pmatrix}
        d_1 & & & \\[5pt]
        & d_2  & & \\[5pt]
        & & \ddots & \\[5pt]
        & & & d_n \\[5pt]
    \end{pmatrix}, \quad
    A=
    \begin{pmatrix}
        c_1 & a_{1,2} & & \\[5pt]
        a_{2,1} & c_2 & \ddots & \\[5pt]
        & \ddots & \ddots & a_{n-1,n} \\[5pt]
        & & a_{n,n-1} & c_n
    \end{pmatrix}.
\end{equation*}

By just computing the matrix product, we get:
\begin{equation}\label{DADinv}
    DAD^{-1}=
    \begin{pmatrix}
        c_1 & \frac{d_1}{d_2}a_{1,2} & & \\[10pt]
        \frac{d_2}{d_1}a_{2,1} & c_2 & \ddots & \\[10pt]
        & \ddots & \ddots & \frac{d_{n-1}}{d_n}a_{n-1,n} \\[10pt]
        & & \frac{d_n}{d_{n-1}}a_{n,n-1} & c_n 
    \end{pmatrix}.
\end{equation}

By imposing that the matrix \(DAD^{-1}\) is symmetric, the following equations are derived:
\begin{align*}
    \left( \frac{d_1}{d_2} \right)^2&=\frac{a_{2,1}}{a_{1,2}},\\[6pt]
    &\vdots\\[5pt]
    \left( \frac{d_{n-1}}{d_n} \right)^2&=\frac{a_{n,n-1}}{a_{n-1,n}}.
\end{align*}

Since \(a_{i,i+1}a_{i+1,i} > 0\), \(i=1,\ldots,n-1\), we can take the square root of the right-hand side to obtain a recursive formula for the \(d_i\)'s:
\begin{align*}
    d_n&=1, \\[6pt]
    d_{i}&=\sqrt{\frac{a_{i+1,i}}{a_{i,i+1}}}\cdot d_{i+1}, \qquad i=n-1,\ldots,1.
\end{align*}

One can easily check that, with this choice for \(D\), the matrix \(DAD^{-1}\) is symmetric by inserting the expressions for \(d_i\) (\(i=1,\ldots,n\)) into Equation \ref{DADinv}.

\end{proof}


==> cartesian/HSWME.tex <==

\section{Two-Dimensional Hyperbolic Shallow Water Moment Equations}

\subsection{Hyperbolicity in multiple dimensions}

First, we need a generalisation of the definition of hyperbolicity to arbitrary dimension. Therefore, the system matrix of the multi-dimensional system has to be defined and this is a bit more involved as in the one-dimensional case

\begin{definition}[multi-dimensional hyperbolicity\cite{koellermeier_dissertation_2017}]\label{multiDHyperbolicity}
A first order, non-linear system of partial differential equations in \(D\) spatial dimensions for \(\mathbf{w}\in\mathbb{R}^n\) and \(\mathbf{A}_i(\mathbf{w})\in\mathbb{R}^{n\times n}\), for \(i=1,\ldots,D\), i.e.
\begin{equation}\label{multi-dimensionalHyperbolicitySystem}
    \mathbf{B}(\mathbf{w})\frac{\partial \mathbf{w}}{\partial t}+\mathbf{A}_i(\mathbf{w})\frac{\partial \mathbf{w}}{\partial x_i}=0,
\end{equation}
is called globally hyperbolic if the matrix \(\mathbf{B}(w)\) is invertible and the system matrix 
\begin{equation}\label{multi-dimensionalSystemMatrix}
\mathbf{A}_{sys}=\left( \mathbf{B}(\mathbf{w}) \right)^{-1}\sum_{i=1}^D\mathbf{A}_i(\mathbf{w})\beta_i,
\end{equation}
for normalized vector \(||\mathbf{\pmb{\beta}}||_2=1\), where \(\mathbf{\beta}=(\beta_1,\ldots,\beta_D)^T\), is diagonalizable with real eigenvalues for every \(\mathbf{w}\in\mathbb{R}^n\).
\end{definition} 

In other words, system \eqref{multi-dimensionalHyperbolicitySystem} is globally hyperbolic if the system matrix \eqref{multi-dimensionalSystemMatrix} is hyperbolic for all directions \(\mathbf{\beta}\) on the unit sphere in \(D\) dimensions. In two dimensions, the system matrix is given by \(\mathbf{A}_{sys}=\beta_1\mathbf{A}_x+\beta_2\mathbf{A}_y\), where \(\beta_1^2+\beta_2^2=1\). In this case, we can think of \(\mathbf{\beta}\) as \((\cos{\theta},\sin{\theta})\). With varying \(\theta \in [0,2\pi[\), this indeed describes a unit circle. Figure \ref{fig:2D} illustrates how the entries of \(\boldsymbol{\beta}\) can be interpreted as a direction.

Further, the system in Definition \ref{multiDHyperbolicity} is \textbf{rotationally invariant} if the system matrix \(\mathbf{A}_{sys}\) does not explicitly depend on the entries of \(\pmb{\beta}\). This is a property that is useful in many applications. It means that waves propagate with the same speed in all directions. It turns out that the Cartesian two-dimensional systems are not rotationally invariant. 

\vspace{1mm}
\begin{figure}[h!]
    \centering
    \begin{tikzpicture}[scale=0.27]
        \draw[step=1cm,lightgray,very thin] (-2.9,-2.9) grid (15.9,7.9);
        \draw[thick,->] (0,0) -- (10.5,0) node[anchor=north west] {\(x\)};
        \draw[thick,->] (0,0) -- (0,6) node[anchor=south east] {\(y\)};
        \draw[->, blue] (0,0) -- (8.3,4.8) node[anchor=south west] {\(\beta_1 A_x + \beta_2 A_y\)};
        \draw[densely dotted, thick] (8.3,4.8) -- (8.3,0) node[anchor=north] {\(\beta_1\)};
        \draw[densely dotted, thick] (8.3,4.8) -- (0,4.8) node[anchor=east] {\(\beta_2\)};
    \end{tikzpicture}
    \caption{Illustration of the system matrix in a two-dimensional system.}
    \label{fig:2D}
\end{figure}

\enlargethispage{3\baselineskip}

Now, we will look at some examples of the 2D SWME. In all examples, it is assumed that the basal topography \(h_b\) is constant and that the vertical axis of the coordinate system is aligned with the negative direction of gravitational acceleration: \(e_x=e_y=0\) and \(e_z=1\).

\subsection{Example: first order system}
The first order system (\(N_x=N_y=1\)) approximates the lateral velocities by a linear polynomial both in the \(x\)-direction and in the \(y\)-direction. Recall the general form of the system \eqref{systemForm}. We will call the system with order \(N_x\) in \(x\)-direction and \(N_y\) in \(y\)-direction the \nomenclature{\((N_x,N_y)\)}{Order \(N_x\) in \(x\)-direction and order \(N_y\) in \(y\)-direction, in Cartesian coordinates}\((N_x,N_y)\)th order system. The conservative fluxes are

\begin{equation*}
    F_x(V) = 
    \begin{pmatrix}
        hu_m \\[5pt]
        \frac{gh^2}{2}+hu_m^2 + \frac{h\alpha_1^2}{3} \\[5pt]
        2hu_m\alpha_1 \\[5pt]
        hu_mv_m+\frac{h\alpha_1 \gamma_1}{3} \\[5pt]
        hv_m\alpha_1+hu_m\gamma_1
    \end{pmatrix}, \qquad
    F_y(V) = 
    \begin{pmatrix}
        hv_m \\[5pt]
        hu_mv_m+\frac{h\alpha_1 \gamma_1}{3} \\[5pt]
        hv_m\alpha_1+hu_m\gamma_1 \\[5pt]
        \frac{gh^2}{2}+hv_m^2 + \frac{h\gamma_1^2}{3} \\[5pt]
        2hv_m\gamma_1
    \end{pmatrix}.
\end{equation*}

\vspace{3mm}

The non-conservative fluxes \(Q_x(V)\) and \(Q_y(V)\) are given by

\vspace{2mm}

\begin{equation*}
    Q_x(V)=
    \begin{pmatrix}
        0 & 0 & 0 & 0 & 0 \\[6pt]
        0 & 0 & 0 & 0 & 0 \\[6pt]
        u_m \alpha_1 & 0 & h u_m & 0 & 0\\[6pt]
        0 & 0 & 0 & 0 & 0 \\[6pt]
        v_m \alpha_1 & 0 & h v_m & 0 & 0
    \end{pmatrix}, \qquad
    Q_y(V)=
    \begin{pmatrix}
        0 & 0 & 0 & 0 & 0 \\[6pt]
        0 & 0 & 0 & 0 & 0 \\[6pt]
        u_m \gamma_1 & 0 & h u_m & 0 & 0\\[6pt]
        0 & 0 & 0 & 0 & 0 \\[6pt]
        v_m \gamma_1 & 0 & h v_m & 0 & 0
    \end{pmatrix}.
\end{equation*}

\vspace{3mm}

We will denote the system matrix of the \((N_x,N_y)\)th order system by \nomenclature{\(A^{(N_x,N_y)}_{sys}\)}{System matrix of the \((N_x,N_y)\)th order Cartesian SWME}\(A^{(N_x,N_y)}_{sys}\). It can be easily verified that the system matrix \(\mathbf{A}^{(1,1)}_{sys}=\beta_1 \mathbf{A}_x^{(1,1)} + \beta_2 \mathbf{A}_y^{(1,1)}\) is given by 

\enlargethispage{1\baselineskip}

\footnotesize
\noindent
\makebox[\textwidth]{\parbox{1.3\textwidth}{
\vspace{7mm}
\begin{equation*}
    \mathbf{A}^{(1,1)}_{sys}=
    \begin{pmatrix}
        u_m\beta_1+v_m\beta_2 & h\beta_1 & 0 & h\beta_2 & 0 \\[7pt]
        g\beta_1+\frac{\alpha_1(\alpha_1\beta_1+\gamma_1\beta_2)}{3h} & u_m\beta_1+v\beta_2 & \frac{1}{3}(2\alpha_1\beta_1+\gamma_1\beta_2) & 0 & \frac{\alpha_1\beta_2}{3} \\[7pt]
        0 & \alpha_1\beta_1+\gamma_1\beta_2 & u_m\beta_1+v_m\beta_2 & 0 & 0 \\[7pt]
        g\beta_2+\frac{\gamma_1(\alpha_1\beta_1+\gamma_1\beta_2)}{3h} & 0 & \frac{\gamma_1\beta_1}{3} & u_m\beta_1+v_m\beta_2 & \frac{1}{3}(\alpha_1\beta_1+2\gamma_1\beta_2) \\[7pt]
        0 & 0 & 0 & \alpha_1\beta_1+\gamma_1\beta_2 & u_m\beta_1+v_m\beta_2
    \end{pmatrix}
\end{equation*}
\vspace{7mm}
}}
\normalsize

A direct computation gives the eigenvalues of \(\mathbf{A}^{(1,1)}_{sys} \in \mathbb{R}^{5\times 5}\):
\begin{align}\label{eigenvalues(1,1)system1}
    \lambda_1&=\beta_1 u_m+\beta_2 v_m,\\[6pt]
    \label{eigenvalues(1,1)system2} \lambda_{2,3}&=\beta_1 u_m+\beta_2 v_m\pm\sqrt{(\beta_1 \alpha+\beta_2 \gamma)^2+gh},\\[6pt]
    \label{eigenvalues(1,1)system3} \lambda_{4,5}&=\beta_1 u_m+\beta_2 v_m\pm\frac{\sqrt{3}}{3}(\beta_1 \alpha+\beta_2 \gamma).
\end{align}

This clearly show that the first order system is not rotationally invariant, because both the system matrix \(\mathbf{A}_{sys}^{(1,1)}\) and the eigenvalues of \(\mathbf{A}_{sys}^{(1,1)}\) depend on the entries of \(\pmb{\beta}\). Intuitively, this is not a surprise. Suppose for example that one is standing in a river. Locally, the water is approximately flowing in one direction in a river. Then one can imagine that one will observe a different velocity profile when the line-of-sight is in alignment with this direction than when the line-of-sight is perpendicular to this direction. So it is certainly not wrong that the Cartesian system is not rotationally invariant. However, it complicates the computations. Can this problem be overcome? In Chapter \ref{ch:HASWME}, we will transform the system to cylindrical coordinates, in the hope to obtain a rotationally invariant system. The intuitive idea is the following. If the system is transformed to cylindrical coordinates (\(r,\theta,\zeta\)), then the potential rotational invariance is explicitly given by the dependence on \(\theta\). This will be discussed in Chapter \ref{ch:HASWME}. In the rest of this chapter, we will keep our focus on the Cartesian SWME and ignore the mathematical complexity that is induced by the dependence of the system matrix on \(\beta_1\) and \(\beta_2\).

\subsection{Hyperbolicity breakdown of SWME}\label{section:hypbreakdown}

Note that the eigenvalues \eqref{eigenvalues(1,1)system1}, \eqref{eigenvalues(1,1)system2} and \eqref{eigenvalues(1,1)system3} are real for all values of \(\beta_1\) and \(\beta_2\) and for all \(V\in \mathbb{R}^{5}\). So the \((1,1)\)th order system is globally hyperbolic. While this is also the case for the first order one-dimensional system, the second order one-dimensional system is not globally hyperbolic, see \cite{SWME} and \cite{HSWME}. We can thus expect that the \((2,2)\)th order system lacks hyperbolicity, too. This is indeed the case. We will look at one particular direction \(\beta_1=1, \beta_2=0\), so we are looking in positive \(x\)-direction. The system matrix is then just \(A_{sys}^{(2,2)}=A_x^{(2,2)}\):

\begin{equation}\label{(2,2)systemMatrix}
    A_{sys}^{(2,2)}=
    \begin{pmatrix}
          0 & 1 & 0 & 0 & 0 & 0 & 0 \\
          d_1 & 2 u_m & \frac{2 \alpha _1}{3} & \frac{2 \alpha _2}{5} & 0 & 0 & 0 \\
          d_2 & 2 \alpha _1 & \alpha _2+u_m & \frac{3 \alpha _1}{5} & 0 & 0 & 0 \\
          d_3 & 2 \alpha _2 & \frac{\alpha _1}{3} & \frac{3 \alpha _2}{7}+u_m & 0 & 0 & 0 \\
          d_4 & v_m & \frac{\gamma _1}{3} & \frac{\gamma _2}{5} & u_m & \frac{\alpha _1}{3} & \frac{\alpha _2}{5} \\
          d_5 & \gamma _1 & \frac{3 \gamma _2}{5} & \frac{\gamma _1}{5} & \alpha _1 & \frac{2 \alpha _2}{5}+u_m & \frac{2 \alpha _1}{5} \\
          d_6 & \gamma _2 & -\frac{\gamma _1}{3} & \frac{\gamma _2}{7} & \alpha _2 & \frac{2 \alpha _1}{3} & \frac{2 \alpha _2}{7}+u_m.
    \end{pmatrix}
\end{equation}

The entries of the first column are not given explicitly to keep the notation light. The full expression can be found in Appendix \ref{ch:hyperbolicityproof(N,N)}. Figure \ref{fig:hypPlot22} shows the lack of hyperbolicity of the second order system. The coefficient \(\gamma_1\) and \(\gamma_2\) are set to zero. Note that the coefficients are scaled. In the red regions, there is a loss of hyperbolicity. 

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.8\textwidth]{image/Chapters/HyperbolicityPlots/(2,2)thOrderHyperbolicityPlot.png}
    \caption{Hyperbolicity plot of the \((2,2)\)th order system with \(\gamma_1,\gamma_2\) set to zero and with \(\beta_1=1,\beta_2=0\). In the red regions, there is a loss of hyperbolicity.}
    \label{fig:hypPlot22}
\end{figure}

\enlargethispage{1\baselineskip}

The hyperbolicity loss occurs for relatively large values of the scaled \(\alpha_1\) and \(\alpha_2\), so it might not be such a big problem in the second order system. On the other hand, the hyperbolicity of the \((3,3)\)th order system, also called the cubic system, is much more severe. This is shown in Figure \ref{fig:hypPlots33}. This figure displays two hyperbolicity plots of the cubic system. In the left panel \ref{fig:hypPlot33_1}, we again look in \(x\)-direction, while in the right panel \ref{fig:hypPlot33_2}, \(\beta_1=\beta_2=\sqrt{2}/2\), which means that we look exactly in between the \(x\)-direction and the \(y\)-direction. Note that in the two scenarios different coefficients are set to zero. In both cases, it can be seen that an infinitesimal deviation from the origin can bring us into a non-hyperbolic region. In other words, already for very small values of the coefficients we can enter a non-hyperbolic region. This is potentially problematic, because these are situations close to equilibrium.

\begin{figure}[h!]
    \centering
    \begin{subfigure}[b]{0.46\textwidth}
        \centering
        \includegraphics[width=\textwidth]{image/Chapters/HyperbolicityPlots/(3,3)thOrderHyperbolicityPlot.png}
        \caption{(3,3)th order system with \(\alpha_2,\gamma_1,\gamma_2,\gamma_3\) set to zero, and with \(\beta_1=1,\beta_2=0\).}
        \label{fig:hypPlot33_1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.46\textwidth}  
        \centering 
        \includegraphics[width=\textwidth]{image/Chapters/HyperbolicityPlots/(3,3)thOrderHyperbolicityPlotCartesian.png}
        \caption{(3,3)th order system with \(\alpha_2,\alpha_3,\gamma_1,\gamma_2\) set to zero, and with \(\beta_1=\beta_2=\frac{\sqrt{2}}{2}\).}
        \label{fig:hypPlot33_2}
    \end{subfigure}
    \caption{Hyperbolicity plots of the \((3,3)\)th order system with different settings for the coefficients and the direction. In the red regions, there is a loss of hyperbolicity.}
    \label{fig:hypPlots33}
\end{figure}

These observations show that the two-dimensional SWME are not globally hyperbolic. Note that the \((2,2)\)th order system and the \((3,3)\)th order system are just examples of the lack of hyperbolicity of the SWME. In general, this does probably not depend on the order \((N_x,N_y)\). It is likely that the \((3,5)\)th order system lacks hyperbolicity too, for example. In the next section, the system will be modified in order to obtain a hyperbolic region. 

\subsection{Hyperbolic Shallow Water Moment Equations}\label{HSWME_Section}


In \cite{HSWME}, hyperbolic shallow water moment equations (HSWME) in one dimension are derived. It was shown that the HSWME were more stable during numerical simulations than the SWME. Also, the one-dimensional SWME turned out to be quite accurate. It is thus a straightforward idea to expand the methodology behind the well-performing HSWME in one dimension to hyperbolic moment equations in two dimensions. In this section, this extension will be discussed. We will see that the analytical derivation of the system is made more complex because of the fact that the Cartesian SWME are not rotationally invariant. Fortunately, an interesting relation will be observed by using the specific structure of the system matrix, making us believe that the resulting system is, in fact, hyperbolic. 

\subsubsection{Modifying the system}
In analogy to the one-dimensional HSWME in \cite{HSWME}, the idea is to linearize the \((N_x,N_y)\)th order system matrix around
\((h,u_m,\alpha_1,0,\ldots,0,v_m,\gamma_1,0,\ldots,0)\), i.e.,
\begin{equation}\label{systemFormHyperbolic}
    (h,u_m,\alpha_1,\ldots,\alpha_{N_x},v_m,\gamma_1,\ldots,\gamma_{N_y})\Longrightarrow (h,u_m,\alpha_1,0,\ldots,0,v_m,\gamma_1,0,\ldots,0).
\end{equation}

So with linearizing we mean that we set the higher order coefficients \(\alpha_i\) \((i=1,\ldots,N_x)\) and \(\gamma_i\) \((i=1,\ldots,N_y)\) to zero. The resulting system of equations is called the two-dimensional \textbf{Hyperbolic Shallow Water Moment Equations (HSWME)} and it has the following form:
\begin{equation*}
    \frac{\partial V}{\partial t} + A_{x,H}(V)\frac{\partial V}{\partial x} + A_{y,H}(V)\frac{\partial V}{\partial y}=S(V).
\end{equation*}

The only difference with \eqref{systemForm} is that the matrices \(A_x\) and \(A_y\) are replaced by the matrices \nomenclature{\(A_{x,H}^{(N,N)}\)}{System matrix of the \((N,N)\)th order Cartesian HSWME, in \(x\)-direction}\(A_{x,H}\) and \nomenclature{\(A_{y,H}^{(N,N)}\)}{System matrix of the \((N,N)\)th order Cartesian HSWME, in \(y\)-direction}\(A_{y,H}\), respectively. The system matrix is now given by:
\begin{equation*}
    A_H = \beta_1A_{x,H} + \beta_2 A_{y,H}, \qquad \beta_1^2 + \beta_2^2 =1.
\end{equation*}
The logical question is: are the HSWME hyperbolic? Hopefully this is the case, otherwise the name of the new system would be rather inconvenient. We know that the one-dimensional HSWME are hyperbolic (\cite{HSWME}), so we have quite a strong belief that the two-dimensional HSWME are hyperbolic, too. But let us first look at an example.  

\subsubsection{Example: (2,2)th order system}
The \((2,2)\)th order system assumes a quadratic vertical velocity profile in both \(x\)- and \(y\)-direction. It has already been observed in Section \ref{section:hypbreakdown} that the two-dimensional quadratic system is not globally hyperbolic. The hyperbolic system matrices \(A_{x,H}^{(2,2)}\) and \(A_{y,H}^{(2,2)}\) are given by

\begin{align*}
    A_{x,H}^{(2,2)}&=
    \begin{pmatrix}
        0 & 1 & 0 & 0 & 0 & 0 & 0 \\[4pt]
        g h-\frac{\alpha _1^2}{3}-u_m^2 & 2 u_m & \frac{2 \alpha _1}{3} & 0 & 0 & 0 & 0 \\[4pt]
        -2 \alpha _1 u_m & 2 \alpha _1 & u_m & \frac{3 \alpha _1}{5} & 0 & 0 & 0 \\[4pt]
        -\frac{2 \alpha _1^2}{3} & 0 & \frac{\alpha _1}{3} & u_m & 0 & 0 & 0 \\[4pt]
        -\frac{\alpha _1 \gamma _1}{3}-u_m v_m & v_m & \frac{\gamma _1}{3} & 0 & u_m & \frac{\alpha _1}{3} & 0 \\[4pt]
         \gamma _1 u_m- \alpha _1 v_m & \gamma _1 & 0 & \frac{\gamma _1}{5} & \alpha _1 & u_m & \frac{2 \alpha _1}{5} \\[4pt]
        -\frac{2}{3} \alpha _1 \gamma _1 & 0 & -\frac{\gamma _1}{3} & 0 & 0 & \frac{2 \alpha _1}{3} & u_m \\[4pt]
    \end{pmatrix}, \\[6pt]
    A_{y,H}^{(2,2)}&=
    \begin{pmatrix}
        0 & 0 & 0 & 0 & 1 & 0 & 0 \\[4pt]
        -\frac{\alpha _1 \gamma _1}{3}-u_m v_m & v_m & \frac{\gamma _1}{3} & 0 & u_m & \frac{\alpha _1}{3} & 0 \\[4pt]
        \gamma _1 u_m- \alpha _1 v_m & \gamma _1 & v_m & \frac{2 \gamma _1}{5} & \alpha _1 & 0 & \frac{\alpha _1}{5} \\[4pt]
        -\frac{2}{3} \alpha _1 \gamma _1 & 0 & \frac{2 \gamma _1}{3} & v_m & 0 & -\frac{\alpha _1}{3} & 0 \\[4pt]
        g h-\frac{\gamma _1^2}{3}-v_m^2 & 0 & 0 & 0 & 2 v_m & \frac{2 \gamma _1}{3} & 0 \\[4pt]
        -2 \gamma _1 v_m & 0 & 0 & 0 & 2 \gamma _1 & v_m & \frac{3 \gamma _1}{5} \\[4pt]
        -\frac{2 \gamma _1^2}{3} & 0 & 0 & 0 & 0 & \frac{\gamma _1}{3} & v_m
    \end{pmatrix}.
\end{align*}

A direct computation of the eigenvalues of \(A_H^{(2,2)} = \beta_1A_{x,H}^{(2,2)} + \beta_2 A_{y,H}^{(2,2)}\) yields:

\begin{align*}
    \lambda_1 &= \beta_1 u_m +\beta_2 v_m, \\[4pt]
    \lambda_{2,3} &= \beta_1 u_m +\beta_2 v_m \pm \sqrt{\frac{1}{5}}(\beta_1 \alpha_1 + \beta_2 \gamma_1), \\[4pt]
    \lambda_{4,5} &= \beta_1 u_m +\beta_2 v_m \pm \sqrt{\frac{3}{5}}(\beta_1 \alpha_1 + \beta_2 \gamma_1), \\[4pt]
    \lambda_{6,7} &= \beta_1 u_m +\beta_2 v_m \pm \sqrt{gh+(\beta_1 \alpha_1 + \beta_2 \gamma_1)^2}.
\end{align*}

The eigenvalues are real, under the restriction that \(h\) is positive. Moreover, if we assume that \(\alpha_1\neq 0 \neq \gamma_1\), then the eigenvalues are distinct. Thus, under these restrictions, we can conclude that the \((2,2)\)th order system of two-dimensional HSWME is globally hyperbolic. The next step is to derive an analytical form of the system matrix of a general \((N_x,N_y)\)th order hyperbolic system. For the one-dimensional hyperbolic systems, this is done in \cite{HSWME}.

\subsubsection{Analytical form of (N,N)th order system matrix}
From now on, we will only focus on the \((N,N)\)th order system, i.e., the systems with equal order in \(x\)- and \(y\)-direction. For this systems, the following theorems are proved. These theorems are some of the main results of my work. The proofs are possible because of the structure of the equations that are derived by using \newglossaryentry{MoM}{name={MoM},description=Method of Moments}\gls{MoM}. This is one of the benefits of the approach of the work. 

\enlargethispage{4\baselineskip}

\begin{theorem}\label{analyticalForm(N,N)}
The hyperbolic Cartesian system matrix \(A_{x,H}^{(N,N)} \in \mathbb{R}^{(2N+3)\times (2N+3)}\) in the \(x\)-direction is given by
\begin{equation}\label{22systemMatrix}
    A_{x,H}^{(N,N)}=
    \begin{pmatrix}
        \mathbf{A}_x^{(N,N)} & \mathbf{0}_x^{(N,N)} \\
        \mathbf{B}_x^{(N,N)} & \mathbf{C}_x^{(N,N)}
    \end{pmatrix},
\end{equation}
where
\footnotesize{
\begin{align*}
    \mathbf{A}_x^{(N,N)}&=
    \begin{pmatrix}
        & 1 & & & &  \\[6pt]
        gh-u_m^2-\frac{1}{3}\alpha_1^2 & 2u_m & \frac{2}{3}\alpha_1 & & & \\[6pt]
        -2 u_m\alpha_1 & 2\alpha_1 & u_m & \frac{3}{5}\alpha_1 & & & \\[6pt]
        -\frac{2}{3}\alpha_1^2 & & \frac{1}{3}\alpha_1 & u_m & \ddots & & \\[6pt]
        & & & \ddots & \ddots & \frac{N+1}{2 N+1}\alpha_1 \\[6pt]
        & & & & \frac{N-1}{2N-1}\alpha_1 & u_m
    \end{pmatrix},\\[10pt]
    \mathbf{B}_x^{(N,N)}&=
    \begin{pmatrix}
        - u_m v_m -\frac{\alpha_1\gamma_1}{3} & v_m & \frac{\gamma_1}{3} & & & \\[6pt]
        -u_m\gamma_1-v_m\alpha_1 & \gamma_1 & v_m & \frac{1}{5}\gamma_1 & & \\[6pt]
        -\frac{2}{3}\alpha_1\gamma_1 & & -\frac{1}{3}\gamma_1 & v_m & \ddots & \\[6pt]
        & & & \ddots & \ddots & \frac{1}{2N+1}\gamma_1 \\[6pt]
        & & & & -\frac{1}{2N-1}\gamma_1 & v_m 
    \end{pmatrix},\\[10pt]
    \mathbf{C}_x^{(N,N)}&=
    \begin{pmatrix}
        u_m & \frac{\alpha_1}{3} & & & & \\[6pt]
        \alpha_1 & u_m & \frac{2}{5}\alpha_1 & & & \\[6pt]
        & \frac{2}{3}\alpha_1 & u_m & \frac{3}{7}\alpha_1 & & \\[6pt]
        & & & \ddots & \ddots & \frac{N}{2N+1}\alpha_1 \\[6pt]
        & & & & \frac{N}{2N-1}\alpha_1 & u_m
    \end{pmatrix},
\end{align*}
}
\vspace{5mm}
\normalsize
with \(\mathbf{A}_x^{(N,N)} \in \mathbb{R}^{(N+2)\times (N+2)}\), \(\mathbf{B}_x^{(N,N)} \in \mathbb{R}^{(N+1)\times (N+2)},\mathbf{C}_x^{(N,N)} \in \mathbb{R}^{(N+1)\times (N+1)}\) and where all other entries are zero. \(\mathbf{0}_x^{(N,N)} \in \mathbb{R}^{(N+2)\times (N+1)}\) is a zero matrix.
\end{theorem}

\begin{proof}
The proof is given in Appendix \ref{ch:hyperbolicityproof(N,N)}. 
\end{proof}

\begin{theorem}
The hyperbolic Cartesian system matrix \(A_{y,H}^{(N,N)} \in \mathbb{R}^{(2N+3)\times (2N+3)}\) in the \(y\)-direction is given by
\begin{equation}
    A_{y,H}^{(N,N)}=
    \begin{pmatrix}
        \mathbf{A}_y^{(N,N)} & \mathbf{D}_y^{(N,N)} \\
        \mathbf{B}_y^{(N,N)} & \mathbf{C}_y^{(N,N)}
    \end{pmatrix},
\end{equation}
where
\footnotesize{
\begin{align*}
    \mathbf{A}_y^{(N,N)}&=
    \begin{pmatrix}
        & & & & &  \\[6pt]
        -u_m v_m -\frac{\alpha_1\gamma_1}{3} & v_m & \frac{\gamma_1}{3} & & & \\[6pt]
        -u_m\gamma_1-v_m\alpha_1 & \gamma_1 & v_m & \frac{2}{5}\gamma_1 & & \\[6pt]
        -\frac{2}3{}\alpha_1\gamma_1 & & \frac{2}{3}\gamma_1 & v_m & \ddots & \\[6pt]
        & & & \ddots & \ddots & \frac{N}{2N+1}\gamma_1 \\[6pt]
        & & & & \frac{N}{2N-1}\gamma_1 & v_m 
    \end{pmatrix},\\[14pt]
    \mathbf{B}_y^{(N,N)}&=
    \begin{pmatrix}
        gh-v_m^2-\frac{1}{3}\gamma_1^2 &  &    \\[6pt]
        -2 v_m\gamma_1 &  &  &   \\[6pt]
        -\frac{2}{3}\gamma_1^2 & &  &     \\[6pt]
        & &    \\[6pt]
        & & 
    \end{pmatrix},\quad
    \mathbf{C}_y^{(N,N)}=
    \begin{pmatrix}
        2v_m & \frac{2}{3}\gamma_1 & & & \\[6pt]
        2\gamma_1 & v_m & \frac{3}{5}\gamma_1 & & & \\[6pt]
         & \frac{1}{3}\gamma_1 & v_m & \ddots & & \\[6pt]
         & & \ddots & \ddots & \frac{N+1}{2 N+1}\gamma_1 \\[6pt]
        & & & \frac{N-1}{2N-1}\gamma_1 & v_m
    \end{pmatrix},\\[14pt]
    \mathbf{D}_y^{(N,N)}&=
    \begin{pmatrix}
        1 & & & & & \\[6pt]
        u_m & \frac{\alpha_1}{3} & & & & \\[6pt]
        \alpha_1 & 0 & \frac{1}{5}\alpha_1 & & & \\[6pt]
        & -\frac{1}{3}\alpha_1 & 0 & \frac{1}{7}\alpha_1 & & \\[6pt]
        & & & & \ddots & \\[6pt]
        & & \ddots & \ddots & \frac{1}{2N+1}\alpha_1 \\[6pt]
        & & & -\frac{1}{2N-1}\alpha_1 & 0
    \end{pmatrix},
\end{align*}
}
\normalsize

%\vspace{5mm}
with \(\mathbf{A}_y^{(N,N)} \in \mathbb{R}^{(N+2)\times (N+2)}\), \(\mathbf{B}_y^{(N,N)} \in \mathbb{R}^{(N+1)\times (N+2)}\), \(\mathbf{C}_y^{(N,N)} \in \mathbb{R}^{(N+1)\times (N+1)}\) and \(\mathbf{D}_y^{(N,N)} \in \mathbb{R}^{(N+2)\times (N+1)}\).
\end{theorem}

\begin{proof}
This can be proved in the exact same way as \ref{analyticalForm(N,N)} is proved, so the proof is not given in this thesis.
\end{proof}

\begin{theorem}
The matrix \(A_{x,H}^{(N,N)}\) of the \((N,N)\)th order HSWME system is diagonalizable with real eigenvalues.
\end{theorem}

\begin{proof}
The proof is given in Appendix
\ref{ch:hyperbolicityproof(N,N)}.
\end{proof}

\begin{theorem}
The matrix \(A_{y,H}^{(N,N)}\) of the \((N,N)\)th order HSWME system is diagonalizable with real eigenvalues.
\end{theorem}

\begin{proof}
The matrix \(A_{y,H}^{(N,N)}\) can be brought in the same form as \(A_{x,H}^{(N,N)}\) by a sequence of permutations of rows and columns. This corresponds to multiplying  \(A_{y,H}^{(N,N)}\) left and right with permutation matrices. The theorems about \(A_{x,H}^{(N,N)}\) in the appendix then also prove this theorem.
\end{proof}

\enlargethispage{1\baselineskip}

The last two theorems are important results, but they are not enough to conclude that the two-dimensional HSWME are hyperbolic. To see this, note that the system matrix of the \((N,N)\)th order hyperbolic system is given by \nomenclature{\(A_H^{(N,N)}\)}{System matrix of the \((N,N)\)th order Cartesian HSWME}\(A_H^{(N,N)}=\beta_1 A_{x,H}^{(N,N)} + \beta_2 A_{y,H}^{(N,N)} \). The sum of two diagonalizable matrices is not necessarily diagonalizable. Since the system matrix explicitly depends on \(\beta_1\) and \(\beta_2\), a computation of the eigenvalues is difficult, even in software such as Mathematica. However, for the systems up to order \((4,4)\), we observe an interesting relation.

\subsubsection{Relation between one-dimensional eigenvalues and two-dimensional eigenvalues}

First of all, note that the eigenvalues of \(A_{x,H}^{(N,N)}\) do not depend on any \(\gamma_j\) (\(j=1,\ldots,N\)) or \(u_m\). Similarly, the eigenvalues of \(A_{y,H}^{(N,N)}\) do not depend on any \(\alpha_j\) (\(j=1,\ldots,N\)) or \(v_m\). The following conjecture formally states our observations.

\enlargethispage{1\baselineskip}

\begin{conjecture}\label{hyp:hyp1}
Denote the characteristic polynomial of \(A_{x,H}^{(N,N)}\) by \(\chi_{A_{x,H}^{(N,N)}}(\lambda;u_m,\boldsymbol{\alpha})\), where we explicitly denoted the dependence on \(u_m\) and \(\boldsymbol{\alpha}\), with \(\boldsymbol{\alpha}=(\alpha_1,\ldots,\alpha_N)\). Denote the characteristic polynomial of \(A_{y,H}^{(N,N)}\) by \(\chi_{A_{y,H}^{(N,N)}}(\lambda;v_m,\boldsymbol{\gamma})\), with \(\boldsymbol{\gamma}=(\gamma_1,\ldots,\gamma_N)\). Denote the characteristic polynomial of \(A_H^{(N,N)}\) by \(\chi_{A_H^{(N,N)}}(\lambda;u_m,v_m,\boldsymbol{\alpha},\boldsymbol{\gamma})\). Denote the domain of \((u_m,v_m,\boldsymbol{\alpha},\boldsymbol{\gamma})\) by \(\Omega\). The following holds:

\begin{align*}
    \chi_{A_{x,H}}(\lambda;\beta_1 \overline{\boldsymbol{\alpha}}+\beta_2\overline{\boldsymbol{\gamma}},\beta_1 \overline{u}_m+\beta_2\overline{v}_m)=\chi_{A_H}(\lambda;\overline{\boldsymbol{\alpha}},\overline{\boldsymbol{\gamma}},\overline{u}_m,\overline{v}_m), \quad  \forall \overline{\boldsymbol{\alpha}},\overline{\boldsymbol{\gamma}},\overline{u}_m,\overline{v}_m \in \Omega, \\[6pt]
    \chi_{A_{y,H}}(\lambda;\beta_1 \overline{\boldsymbol{\alpha}}+\beta_2\overline{\boldsymbol{\gamma}},\beta_1 \overline{u}_m+\beta_2\overline{v}_m)=\chi_{A_H}(\lambda;\overline{\boldsymbol{\alpha}},\overline{\boldsymbol{\gamma}},\overline{u}_m,\overline{v}_m), \quad \forall \overline{\boldsymbol{\alpha}},\overline{\boldsymbol{\gamma}},\overline{u}_m,\overline{v}_m \in \Omega.
\end{align*}
\end{conjecture}

This can be interpreted in the following way: if we compute the characteristic polynomial of \(A_{x,H}^{(N,N)}\), and then apply the transformation
\begin{equation}
    \boldsymbol{\alpha}\to \beta_1\boldsymbol{\alpha}+\beta_2\boldsymbol{\gamma},
\end{equation}
we obtain the characteristic polynomial of \(A_H^{(N,N)}\) and an analogous statement is true for \(A_{y,H}^{(N,N)}\). 

\paragraph{Example of this relation.} Consider the \((1,1)\)th order system. The characteristic polynomials of the matrices \(A_{x,H}^{(1,1)}\), \(A_{y,H}^{(1,1)}\) and \(A_H^{(1,1)}\) are given by

\begin{multline*}
    \qquad \quad \qquad \chi_{A_{x,H}^{(1,1)}}(\lambda;\alpha_1)=-\lambda^5 + \left(\frac{4 \textcolor{red}{\alpha _1}^2}{3}+1\right) \lambda ^3+\left(-\frac{\alpha _1^4}{3}-\frac{\alpha _1^2}{3}\right) \lambda, \\[6.5pt]
    \chi_{A_{y,H}^{(1,1)}}(\lambda;\gamma_1)=-\lambda^5 + \left(\frac{4 \textcolor{red}{\gamma _1}^2}{3}+1\right) \lambda ^3+\left(-\frac{\gamma _1^4}{3}-\frac{\gamma _1^2}{3}\right) \lambda,  \\[6.5pt]
    \chi_{A_{sys,H}^{(1,1)}}(\lambda;\alpha_1,\gamma_1)=-\lambda^5 + \left(\frac{4 \textcolor{red}{(\beta_1 \alpha_1 + \beta_2\gamma_1)}^2}{3}+1\right) \lambda ^3+\\ \qquad \qquad\left(-\frac{(\beta_1 \alpha_1 + \beta_2\gamma_1)^4}{3}-\frac{(\beta_1 \alpha_1 + \beta_2\gamma_1)^2}{3}\right) \lambda,
\end{multline*}

respectively. Some parts are colored red in the expressions to illustrate the relation. One can see that the described relation holds. Since this is true for the characteristic polynomials, it is also true for the eigenvalues:

\begin{equation*}
    \sigma(A_{x,H}^{(1,1)}) = \{ u_m,u_m\pm\sqrt{\textcolor{red}{\alpha_1}^2+gh},
    u_m\pm\frac{\sqrt{3}}{3}\alpha_1  \},
\end{equation*}

\begin{equation*}
    \sigma(A_{y,H}^{(1,1)}) = \{ v_m,v_m\pm\sqrt{\textcolor{red}{\gamma_1}^2+gh},
    v_m\pm\frac{\sqrt{3}}{3}\gamma_1  \},
\end{equation*}

\begin{multline*}
    \qquad \qquad \qquad \sigma(A_{sys}^{(1,1)})= \{
    \beta_1 u_m+\beta_2 v_m,
    \beta_1 u_m+\beta_2 v_m\pm\sqrt{\textcolor{red}{(\beta_1 \alpha_1+\beta_2 \gamma_1)}^2+gh}, \\
    \beta_1 u_m+\beta_2 v_m\pm\frac{\sqrt{3}}{3}(\beta_1 \alpha_1+\beta_2 \gamma_2) \}.
\end{multline*}


In particular, this would mean that the two-dimensional HSWME are hyperbolic. This follows from the specific form of the eigenvalues of \(A_{x,H}^{(N,N)}\) and \(A_{y,H}^{(N,N)}\), see Appendix \ref{ch:hyperbolicityproof(N,N)}.

\begin{conjecture}
the \((N,N)\)th order system of the HSWME \eqref{systemFormHyperbolic} is globally hyperbolic \(\forall N \in \mathbb{N}\).
\end{conjecture}

The difficulty in proving this is the dependence of the system matrix on \(\beta_1\) and \(\beta_2\), making the calculations tedious. However, we believe that proving \eqref{hyp:hyp1} is doable, such that it is an interesting suggestion for future work. 





==> cartesian/Introduction.tex <==

\section{Introduction}

In \cite{SWME} and \cite{HSWME}, it is observed that the one-dimensional SWME lack global hyperbolicity. The loss of hyperbolicity can lead to unphyiscal oscillations in numerical simulations. Further, hyperbolicity also guarantees that the propagation speeds of the systems are finite. In our situation, we want propagation speeds with non-zero imaginary part, because otherwise, information could travel with infinite or imaginary velocity. Thus, hyperbolicity is an important property of some partial differential equations and we would prefer our systems to be hyperbolic. The drawback of this is that our system has to be modified in order to make it hyperbolic, which can result in a system that is less accurate. Thus, there is a trade-off between hyperbolicity and accuracy. Since for some applications, importance is attached to finite propagation speeds and more stable numerical simulations, hyperbolic shallow water moment models in one dimension were developed in \cite{HSWME}. In this chapter, we will extend the one-dimensional models to two dimensions, in the hope to derive hyperbolic models that can be used to model two-dimensional flow.



==> cartesian/Numerics.tex <==

\section{Numerical simulation}\label{numerics}

The systems (SWME and HSWME) were implemented in C++ to do numerical simulations. The code was provided by Dr. Julian Koellermeier \cite{koellermeier_dissertation_2017}. The goal was to find a test case such that the simulations using the SWME show unphysical oscillations, while the HSWME show stable and accurate results. This is inspired by the numerical results in \cite{HSWME}. Both smooth test cases and dam break problems were considered. Note that the numerical schemes are not discussed here. A detailed study on numerical schemes for shallow water moment equations can be a Master's thesis on itself. For example, in this thesis it is assumed in the simulations that the bottom topography \(h_b\) is constant in space, such that \(\partial_x h_b\) and \(\partial_y h_b\) are equal to zero in \eqref{projectedXMomentum} and \eqref{projectedYMomentum}. In \cite{koellermeier_steady_2022}, well-balanced schemes with topology are obtained, such that it is not assumed that \(h_b=constant\). However, this is beyond the scope of this thesis.

\subsection{Used numerical schemes and grid}
Since we are dealing with systems of non-conservative PDEs, we use the PRICE scheme with forward Euler time integration. An overview of finite volume schemes and in particular the PRICE scheme is given in \cite{koellermeier_dissertation_2017}. In all of the numerical simulations with Cartesian systems, the same grid is used, namely a 100 by 100 square grid. The two-dimensional domain is \([0,1]\times [0,1]\). Thus, we have, with \(\Delta x=\Delta_y=0.01\):
\begin{align*}
    x_i &= i \Delta x, \qquad i=0,\ldots,100, \\[5pt]
    y_i &= i \Delta y, \qquad i=0,\ldots,100.
\end{align*}
The boundary of each cell is composed of four faces with the same length. Apart from the boundary cells, each cell has four direct neighbour cells. Further, the domain is periodic, meaning that what flows out through the right boundary comes in through the left boundary (and vice versa) and what flows out through the bottom boundary flows in through the top boundary (and vice versa).

\subsection{Simulation of a smooth Gaussian}

\enlargethispage{2\baselineskip}

First, a test case with a smooth Gaussian as initial height function is considered. Figure \ref{fig:initialHeight_gaussian} shows the height profile at time zero. The initial value of the lateral velocities and the coefficients are all zero. The \((3,3)\)th order system is used. The setup for the test case is given in Table \ref{table:smoothGaussian}. 

\begin{table}[h!]
\begin{tabular}{ | m{9em} || m{6cm} | } 
  \hline
  Order & \((3,3)\) \\[4pt]
  \hline
  \(\nu\) & \(\nu=0.1\) \\[4pt] 
  \hline
  \(\lambda\) & \(\lambda=0.01\) \\[4pt]
  \hline
  Spatial domain & \(x\in [0,1], \quad y \in [0,1]\) \\[4pt]
  \hline
  \(h(x,y,0)\) & \(1+\frac{1}{20}\cdot \frac{\exp(-\frac{1}{2}\left(\left(\frac{x-0.5}{0.2} \right)^2+\left(\frac{y-0.5}{0.2} \right)^2\right))}{0.08\pi}\) \\[8pt] 
  \hline
  \(u(x,y,\zeta,0)\) & \(u(x,y,\zeta,0)=0\) \\[4pt]
  \hline
  \(v(x,y,\zeta,0)\) & \(v(x,y,\zeta,0)=0\)\\[4pt]
  \hline
  Time integration & Forward Euler \\[4pt]
  \hline
  Spatial discretization & PRICE scheme \\[4pt]
  \hline
\end{tabular}
\caption{Simulation set up for smooth Gaussian test case.}
\label{table:smoothGaussian}
\end{table}

The end time of the simulation is \(t_{end}=1.5\). The results are displayed in Figure \ref{fig:smoothGaussian}. The curves in Figure \ref{fig:height_gaussian}-\ref{fig:halpha3_gaussian} correspond to the values along the white line that is shown in \ref{fig:initialHeight_gaussian}. The \(x\)-axis in Figure \ref{fig:height_gaussian}-\ref{fig:halpha3_gaussian} is the distance along this line, i.e., \(d=\sqrt{x^2+y^2}\).

\begin{figure}[h!]
    \centering
    \begin{subfigure}[b]{0.41\textwidth}
        \centering
        \includegraphics[width=\textwidth]{image/Chapters/NumericalSimulation_Cartesian/SmoothGaussian/InitialHeight.png}
        \caption{\(h(x,y,0)\)}
        \label{fig:initialHeight_gaussian}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.41\textwidth}  
        \centering 
        \begin{overpic}[width=\textwidth]{image/Chapters/NumericalSimulation_Cartesian/SmoothGaussian/h.png}
            \put(-16,120){\scriptsize{\(h\)}}
            \put(135,-7){\tiny{\(\sqrt{x^2+y^2}\)}}
        \end{overpic}
        \caption{\(h\) at time \(t=1.5\)}
        \label{fig:height_gaussian}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{0.41\textwidth}   
        \centering 
        \begin{overpic}[width=\textwidth]{image/Chapters/NumericalSimulation_Cartesian/SmoothGaussian/hum.png}
            \put(-16,120){\scriptsize{\(hu_m\)}}
            \put(135,-7){\tiny{\(\sqrt{x^2+y^2}\)}}
        \end{overpic}
        \caption{\(hu_m\) at time \(t=1.5\)}
        \label{fig:hum_gaussian}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.41\textwidth}   
        \centering 
        \begin{overpic}[width=\textwidth]{image/Chapters/NumericalSimulation_Cartesian/SmoothGaussian/halpha1.png}
            \put(-16,120){\scriptsize{\(h\alpha_1\)}}
            \put(135,-7){\tiny{\(\sqrt{x^2+y^2}\)}}
        \end{overpic}
        \caption{\(h\alpha_1\) at time \(t=1.5\)}
        \label{fig:halpha1_gaussian}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{0.41\textwidth}   
        \centering 
        \begin{overpic}[width=\textwidth]{image/Chapters/NumericalSimulation_Cartesian/SmoothGaussian/hgamma2.png}
            \put(-16,120){\scriptsize{\(h\gamma_2\)}}
            \put(135,-7){\tiny{\(\sqrt{x^2+y^2}\)}}
        \end{overpic}
        \caption{\(h\gamma_2\) at time \(t=1.5\)}
        \label{fig:hgamma2_gaussian}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.41\textwidth}   
        \centering 
        \begin{overpic}[width=\textwidth]{image/Chapters/NumericalSimulation_Cartesian/SmoothGaussian/halpha3.png}
            \put(-16,120){\scriptsize{\(h\alpha_3\)}}
            \put(135,-7){\tiny{\(\sqrt{x^2+y^2}\)}}
        \end{overpic}
        \caption{\(h\alpha_3\) at time \(t=1.5\)}
        \label{fig:halpha3_gaussian}
    \end{subfigure}
    \caption{Test case with smooth Gaussian initial height profile for SWME (red curves) and HSWME (blue curves) and \(t=1.5\). The SWME and the HSWME produce almost identical results.}
    \label{fig:smoothGaussian}
\end{figure}
\clearpage

The SWME and the HSWME produce very similar simulations. The curves for the height at time 1.5 in \ref{fig:height_gaussian} are almost indistinguishable. Only by zooming in, one would be able to see a difference. For the other variables, the differences are minor, too. There are three remarks about Figure \ref{fig:smoothGaussian}. The first one is about the missing of some of the coefficients. This is because of the symmetry: the curve for \(h\gamma_1\) is the same as the curve for \(h\alpha_1\), for example. Secondly, the values for \(hu_m,h\alpha_1,h\gamma_2\) and \(h\alpha_3\) are given and not the values of \(u_m,\alpha_1,\gamma_2\) and \(\alpha_3\). This is because in the implementation in C++, the equations are solved in so-called convective variables \(h,hu_m,h\alpha_1,\ldots\) and not in primitive variables \(h,u_m,\alpha_1,\ldots\). The third remark is that the accuracy of the SWME and HSWME is not really illustrated in \ref{fig:smoothGaussian}, because there is no reference solution. This is an important suggestion for future work. Now, it is difficult to tell something meaningful about the accuracy.   

\subsection{Discontinuous initial height profile}
In the smooth test case discussed in the previous section, SWME and HSWME gave very similar results. We will now see if this is also the case for a discontinuous initial height function. On top of the comparison between SWME and HSWME, systems of different order will be compared. Table \ref{table:damBreakSquare} gives the setup for this numerical test case. The initial lateral velocities are chosen such that we theoretically start in a non-hyperbolic region.

\begin{table}[h!]
\begin{tabular}{ | m{9em} || m{6cm} | } 
  \hline
  \(\nu\) & \(\nu=0.1\) \\[4pt] 
  \hline
  \(\lambda\) & \(\lambda=0.01\) \\[4pt]
  \hline
  Spatial domain & \(x\in [0,1], \quad y \in [0,1]\) \\[4pt]
  \hline
  \(h(x,y,0)\) & \[
                    h(x,y,0) = \left\{\begin{array}{lr}
                    5, &  0.25 \leq x,y \leq 0.75 \\ 
                    1, &  \text{everywhere else}
                    \end{array} \right.
                \] \\[4pt] 
  \hline
  \(u(x,y,\zeta,0)\) & \(u(x,y,\zeta,0)=-3.6\zeta^3+5.4 \zeta^2 -1.66\zeta +0.18\) \\[4pt]
  \hline
  \(v(x,y,\zeta,0)\) & \(v(x,y,\zeta,0)=-3.6\zeta^3+5.4 \zeta^2 -1.66\zeta +0.18\)\\[4pt]
  \hline
  Time integration & Forward Euler \\[4pt]
  \hline
  Spatial discretization & FORCE scheme \\[4pt]
  \hline
\end{tabular}
\caption{Simulation set up for discontinuous test case.}
\label{table:damBreakSquare}
\end{table}

\enlargethispage{2\baselineskip}

The numerical results are shown in Figure \ref{fig:damBreakSquare}. The initial height profile is illustrated in \ref{fig:initialHeight_damBreakSquare}. Again, the line along which the values of the functions are plotted is illustrated. Figure \ref{fig:height_damBreakSquare} gives the height of the flow at time \(t=1.0\) for order \((0,0)\), i.e., the shallow water equations, up to order (3,3) and for the (3,3)th order hyperbolic system. At this time, the waves have already interacted with each other, because of the periodic domain. Clearly, there are big differences between the different orders. The (0,0)th order system and the (1,1)th order system result in very different heights than the (2,2)th order system and both (3,3)th order systems. The SWE also stand out when it comes to the simulation of \(hu_m\) and \(hv_m\) as shown in Figure \ref{fig:hum_damBreakSquare} and \ref{fig:hvm_damBreakSquare}, respectively. However, due to the convective form of the variables, the differences observed in the height \(h\) is also transported into \(hu_m\) and \(hv_m\). For a fair comparison, it is necessary to extract the primitive variables from the output.

When we specifically look at the (3,3)th order SWME and the (3,3)th order HSWME, we observe that the differences in height \(h\) and lateral velocities \(u_m\) and \(v_m\) are small. Figure \ref{fig:halpha2_damBreakSquare} displays the values for \(h\alpha_2\) for SWME and HSWME. Here, the differences look bigger, but the scale of the y-axis is much smaller. The same can be observed in Figure \ref{fig:hgamma3_damBreakSquare}, in which the values of \(h\gamma_3\) are plotted. Since these differences are small in absolute sense, they do not cause big differences in the height or velocity profile. No reference solution is implemented, yet, such that making statements about the accuracy of the systems is difficult. In Figure \ref{fig:endHeights}, the height profile of the water at time \(t_{end}=1.0\) is shown, for the different models. 

An important observation is that there are no instabilities in the simulations with the SWME, despite starting in a non-hyperbolic region. This was the case in all numerical simulations: multiple initial conditions and lots of values for the friction parameters were considered, yet no instabilities were found. One of the possible explanations for this is that the PRICE scheme is very stable. Further, the choice of friction parameters may be very sensitive, which means that very specific values need to be chosen in order to find instability. Thus, it is important to realize that in theory, it is possible to encounter unphyscial oscillations in numerical simulations, but this depends on a lot of factors. The fact that we did not encounter instabilities does not mean that the SWME are always stable.     

A last remark is that only simulations with \((N,N)\)th order systems are implemented. This means that there is no flexibility in letting the orders in \(x\)-direction and in \(y\)-direction be different. There are situations in which this is not very appropriate. In a river, the water is typically flowing much more in one direction than in the other. In such a scenario, we might want a simulation in which the approximation of the flow in the main direction has a higher order than in the other direction. The advantage of this is that the \((5,1)\)th order system is faster to simulate than the \((5,5)\)th order system, for example.  

\begin{figure}[h!]
    \centering
    \begin{subfigure}[b]{0.42\textwidth}
        \centering
        \includegraphics[width=\textwidth]{image/Chapters/NumericalSimulation_Cartesian/DamBreakSquare/InitialHeight.png}
        \caption{\(h(x,y,0)\)}
        \label{fig:initialHeight_damBreakSquare}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.42\textwidth}  
        \centering 
        \begin{overpic}[width=\textwidth]{image/Chapters/NumericalSimulation_Cartesian/DamBreakSquare/h.png}
            \put(-16,120){\scriptsize{\(h\)}}
            \put(135,-7){\tiny{\(\sqrt{x^2+y^2}\)}}
        \end{overpic}
        \caption{\(h\) at time \(t=1.0\)}
        \label{fig:height_damBreakSquare}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{0.42\textwidth}   
        \centering 
        \begin{overpic}[width=\textwidth]{image/Chapters/NumericalSimulation_Cartesian/DamBreakSquare/hum.png}
            \put(-16,120){\scriptsize{\(hu_m\)}}
            \put(135,-7){\tiny{\(\sqrt{x^2+y^2}\)}}
        \end{overpic}
        \caption{\(hu_m\) at time \(t=1.0\)}
        \label{fig:hum_damBreakSquare}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.42\textwidth}   
        \centering 
        \begin{overpic}[width=\textwidth]{image/Chapters/NumericalSimulation_Cartesian/DamBreakSquare/hvm.png}
            \put(-16,120){\scriptsize{\(hv_m\)}}
            \put(135,-7){\tiny{\(\sqrt{x^2+y^2}\)}}
        \end{overpic}
        \caption{\(hv_m\) at time \(t=1.0\)}
        \label{fig:hvm_damBreakSquare}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{0.42\textwidth}   
        \centering 
        \begin{overpic}[width=\textwidth]{image/Chapters/NumericalSimulation_Cartesian/DamBreakSquare/halpha2.png}
            \put(-16,120){\scriptsize{\(h\alpha_2\)}}
            \put(135,-7){\tiny{\(\sqrt{x^2+y^2}\)}}
        \end{overpic}
        \caption{\(h\alpha_2\) at time \(t=1.0\)}
        \label{fig:halpha2_damBreakSquare}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.42\textwidth}   
        \centering 
        \begin{overpic}[width=\textwidth]{image/Chapters/NumericalSimulation_Cartesian/DamBreakSquare/hgamma3.png}
            \put(-16,120){\scriptsize{\(h\gamma_3\)}}
            \put(135,-7){\tiny{\(\sqrt{x^2+y^2}\)}}
        \end{overpic}
        \caption{\(h\gamma_3\) at time \(t=1.0\)}
        \label{fig:hgamma3_damBreakSquare}
    \end{subfigure}
    \caption{Test case with discontinuous initial height profile for different orders \((N,N)\) and the (3,3)th order HSWME at time \(t=1.0\). There are big differences between the \((0,0)\)th order system and the higher order systems. The difference between the (3,3)th order SWME and the (3,3)th order HSWME is small.}
    \label{fig:damBreakSquare}
\end{figure}


\begin{figure}[h!]
    \centering
    \begin{subfigure}{.42\textwidth}
        \includegraphics[width=\textwidth]{image/Chapters/NumericalSimulation_Cartesian/DamBreakSquare/EndHeight_SWE.png}
        \caption{(0,0)th order system (SWE)}
        \label{fig:height_endTime_SWE}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.42\textwidth}
        \includegraphics[width=\textwidth]{image/Chapters/NumericalSimulation_Cartesian/DamBreakSquare/EndHeight_11_SWME.png}
        \caption{(1,1)th order SWME}
        \label{fig:height_endTime_11}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}{.42\textwidth}
        \includegraphics[width=\textwidth]{image/Chapters/NumericalSimulation_Cartesian/DamBreakSquare/EndHeight_22_SWME.png}
        \caption{(2,2)th order SWME}
        \label{fig:height_endTime_22}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.42\textwidth}
        \includegraphics[width=\textwidth]{image/Chapters/NumericalSimulation_Cartesian/DamBreakSquare/EndHeight_33_SWME.png}
        \caption{(3,3)th order SWME}
        \label{fig:height_endTime_33_SWME}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}{.42\textwidth}
        \includegraphics[width=\textwidth]{image/Chapters/NumericalSimulation_Cartesian/DamBreakSquare/EndHeight_33_HSWME.png}
        \caption{(3,3)th order HSWME}
        \label{fig:height_endTime_33_HSWME}
    \end{subfigure}
    \caption{3D plot of \(h\) at time \(t=1.0\) for the different models. There are clear differences visible between systems of different order. The difference between (3,3)th order SWME (d) and (3,3)th order HSWME (e) is small.}
    \label{fig:endHeights}
\end{figure}

\clearpage
